Fast Multiple Pattern Cartesian Tree Matching

Cartesian tree matching is the problem of finding all substrings in a given text which have the same Cartesian trees as that of a given pattern. In this paper, we deal with Cartesian tree matching for the case of multiple patterns. We present two fingerprinting methods, i.e., the parent-distance encoding and the binary encoding. By combining an efficient fingerprinting method and a conventional multiple string matching algorithm, we can efficiently solve multiple pattern Cartesian tree matching. We propose three practical algorithms for multiple pattern Cartesian tree matching based on the Wu-Manber algorithm, the Rabin-Karp algorithm, and the Alpha Skip Search algorithm, respectively. In the experiments we compare our solutions against the previous algorithm [18]. Our solutions run faster than the previous algorithm as the pattern lengths increase. Especially, our algorithm based on Wu-Manber runs up to 33 times faster.

==> exp_grouping.tex <==
\begin{figure}[H]
    \centering

    \begin{subfigure}[b]{0.65\textwidth}
        \includegraphics[width=\linewidth]{figures/equal_length_k10_nogroup.png}
        \caption{k=10}
        \label{fig:exp_equal_length_k10}
    \end{subfigure}
    \begin{subfigure}[b]{0.65\textwidth}
        \includegraphics[width=\linewidth]{figures/equal_length_k50_nogroup.png}
        \caption{k=50}
        \label{fig:exp_equal_length_k50}
    \end{subfigure}
    \begin{subfigure}[b]{0.65\textwidth}
        \includegraphics[width=\linewidth]{figures/equal_length_k100_nogroup.png}
        \caption{k=100}
        \label{fig:exp_equal_length_k100}
    \end{subfigure}
    
    \caption{Evaluation on the equal length patterns without grouping technique}
    \label{fig:exp_equal_length}
\end{figure}
